Open-World Instance Segmentation: Exploiting Pseudo Ground Truth From Learned Pairwise Affinity

Open-world instance segmentation is the task of grouping pixels into object instances without any pre-determined taxonomy. This is challenging, as state-of-the-art methods rely on explicit class semantics obtained from large labeled datasets, and out-of-domain evaluation performance drops significantly. Here we propose a novel approach for mask proposals, Generic Grouping Networks (GGNs), constructed without semantic supervision. Our approach combines a local measure of pixel affinity with instance-level mask supervision, producing a training regimen designed to make the model as generic as the data diversity allows. We introduce a method for predicting Pairwise Affinities (PA), a learned local relationship between pairs of pixels. PA generalizes very well to unseen categories. From PA we construct a large set of pseudo-ground-truth instance masks; combined with human-annotated instance masks we train GGNs and significantly outperform the SOTA on open-world instance segmentation on various benchmarks including COCO, LVIS, ADE20K, and UVO. Code is available on project website: https://sites.google.com/view/generic-grouping/.

==> latex/discussion.tex <==
\section{Discussion}

\textbf{Combine grouping and recognition.} With one step forward in grouping pixels in the open-world by \Our{}, we take a step back and ask how \Our{} can be adopted when both grouping and recognition are required. 

As a proof of concept, we use a two-tower module for class-aware instance segmentation: a grouping module (\Our{}) and a recognition module (Mask R-CNN). The grouping module outputs bounding boxes and masks as input to the recognition module, and recognition module classify the boxes and masks. Grouping module is fixed during training of recognition module, and no altering or refinement is given for the grouping results during inference. \Our{} is trained on VOC masks only. We compare this with end-to-end Mask R-CNN in limited data domain: 10\% of COCO images on all classes. Whereas Mask R-CNN is trained on grouping from all categories, the two-tower grouping module only leverages VOC masks and generated pseudo masks. 

\begin{table}[t]
\captionsetup{font=footnotesize}
  \centering
  {\small
  \begin{tabular}{|c|c|c|c|}
    \hline
    Training length & Method & mAP & mAR  \\
    \hline
    \multirow{2}{*}{short} & Mask R-CNN & 10.6 & 36.2 \\
     & Two-Tower & \textbf{12.7} & \textbf{36.5} \\
    \hline
    \multirow{2}{*}{normal} & Mask R-CNN & \textbf{15.4} & \textbf{40.0} \\
     & Two-Tower & 13.5 & 36.5 \\
    \hline
  \end{tabular}}
  \caption{\textbf{Proof of concept on Two-Tower model for grouping and recognition} Mask R-CNN is trained on all 80 COCO categories. \Our{}, as the grouping module, is only trained on 20 VOC classes. The recognition module does not alter the mask predictions of the grouping module, and is trained with 80 COCO categories for classification. Two-tower is competitive in both short and normal training schedules.}
  \label{tab:two_tower}
\end{table}

==> latex/experiments.tex <==
\section{Experiments}
\label{sec:experients}

\subsection{Open-world instance segmentation is hard}
\begin{enumerate}
\item gaps between seen vs. unseen when increasing taxonomies: person -- VOC -- LVIS.
\item trade-offs between seen vs. unseen wrt initial learning rates.
\end{enumerate}
\subsection{Ablation study}

\subsection{Open-world instance segmentation with \Ours{}}

\subsection{Understanding \Ours{}}


==> latex/intro.tex <==
\section{Introduction}
\label{sec:intro}

%\begin{figure}
%  \centering
%    \includegraphics[width=0.9\linewidth]{latex/images/teaser.pdf}
%  \caption{{\bf Generic region proposals are essential for open-world instance detection}. (a) an image (from ADE20K~\cite{}) with ground truth object masks overlaid with different colors. Three different approaches: (b) Selective Search (SS)~\cite{SelectiveSearch}, (b) Mask R-CNN~\cite{8237584}, and (c) our Generic Grouping Network (\Our{}) is applied on the same image and returned the top $100$ proposals. The number of true positive detections or ground truth objects are denoted in parentheses. Among 20 ground truth objects, SS recalls only 1, Mask R-CNN detects 5, and \Our{} retrieves 10. SS is a bottom-up non-parametric approach, thus has no notion of parts or objects. Mask R-CNN can make whole object proposal prediction; however it still fails to detect unseen objects due to being biased to seen classes during top-down training. Our \Our{} can predict full object proposals and is generalized well to unseen classes.}
%  \label{fig:intro}
%\end{figure}

%Story flow looks like:
%\begin{enumerate}
%    \item briefly describe open-world instance segmentation and what make it hard?
%    \item current SoTA top-down methods are biased to seen classes while bottom-up traditional approaches have no notion of part/object boundaries but local, greedy, hand-designed rule-based grouping.
%    \item can we combine the best of both worlds? We propose an approach for proposing generic regions: Generic Proposal Networks (GPN) for open-world instance segmentation by using both bottom-up grouping and top-down training.
%\end{enumerate}

Instance segmentation is the task of grouping pixels into object instances~\cite{8237584}. In the traditional setup, a.k.a closed-world, the model learns to detect and segment objects from a predefined taxonomy. % during both training and testing. 
In contrast, the open-world setting requires the model to segment objects of arbitrary categories. For a model trained in the traditional setup, this means segmenting not only the ``seen'' categories (those presented at training time) but also the ``unseen'' categories (not seen during training)~\cite{uvo,oln}. There is generally a large performance gap between the seen and unseen domains. For example, we compare Average Recall (AR@100) of Mask R-CNN~\cite{8237584} trained on 80 COCO~\cite{Lin2014MicrosoftCC} classes vs a subset of 20 classes. AR@100 of 60 classes out of training taxonomy drops from $49.6\%$ to $19.9\%$ when no mask of these classes is provided in training data (Table~\ref{tab:diff_setup}). The ``unseen'' gap is still large if we train on larger taxonomy (e.g., 1,000+ classes in training data Table~\ref{tab:diff_setup}, please refer to section~\ref{sec:cross_category} for more details).

%\mdf{I find table 5 difficult to map to the experiments described here} \WW{Is it because table 5's header is upper bound? and Upper bound is not very clear yet here.} \mdf{Yes, in part; I think table 5 also just has a lot going on in addition to the points made here.} \WW{I tried to rephrase a bit to avoid going into too many details, but maybe we can say something like ``please refer to sec.4 for more details?"}\DT{this also works as we do not want to go off the flow of the main story.}

%When adapting the current state-of-the-art model, e.g., Mask R-CNN~\cite{8237584}, from closed-world to open-world setup, the performance gaps between these two problem setups are large: Average Recall (AR100) is dropped by an absolute $29.7\%$ from $49.6\%$ (train and evaluate on all 80 COCO categories) to $19.9\%$ (train on only 20 VOC classes and evaluate on the other 60 non-VOC classes from COCO) as shown in Table~\ref{tab:diff_setup}. The gaps are still consistently large even with larger training taxonomy, e.g., using more than 1,000 LVIS~\cite{8954457} categories for training (Table~\ref{tab:diff_setup}). 

%In real applications, open-world instance segmentation can be even harder due to the unknown trade-off of seen and unseen categories during training and real deployment time. Figure~\ref{fig:tradeoff} shows the AR100 of a class-agnostic Mask R-CNN trained under two different seen/unseen splits of COCO: Person vs. non-Person or VOC vs. non-VOC classes. In both settings, there is a clear trade-off in performance of seen and unseen categories we vary the base learning rate. We note that one can only optimize for seen classes during training and validation since the unseen classes are not available until real testing or deployment. Furthermore, this uncertain seen/unseen trade-off can be significantly different across different applications: e.g., the frequencies of encountering novel objects in different applications are different.


%\begin{figure}
%\centering
%\captionsetup{font=footnotesize}
%{\small 
% \begin{subfigure}[b]{0.49\linewidth}
%    {\includegraphics[width=\linewidth]{./images/Person_tradeoff.pdf}}
%    \caption{}
% \end{subfigure}
% \begin{subfigure}[b]{0.49\linewidth}
%    {\includegraphics[width=\linewidth]{./images/VOC_tradeoff.pdf}}
%    \caption{}
% \end{subfigure}
% \label{fig:tradeoff}
% \caption{{\bf The performance trade-off between seen and unseen objects in open-world instance segmentation}. A class-agnostic Mask R-CNN is adopted to two open-world setups: (a) train on Person (seen) and evaluate on non-Person masks (unseen); (b) train on VOC classes (seen) and evaluate on non-VOC (unseen). The plots show the performance (in AR100 metric) for both seen and unseen classes when the base learning rate is varying from $0.01$ to $0.08$. There is a clear trade-off between seen and unseen classes in term of performance, and unfortunately this trade-off can only be revealed during deployment and cannot be addressed by validation.\DT{TODO: re-render plots with seen and unseen text in axis label. AR100 can be removed as captions cover it already.}
%\Heng{These two figures may raise more questions instead of being used as motivation. The first impression to the reviewers is that our method is very sensitive to the learning rate. BTW, we need to explain what the base learning rate is, or use the real learning rate instead. Second, when base learning rate changes from 0.01 to 0.02, both seen and unseen AR are improved. This doesn't help our argument. I suggest to do the following experiments that may serve our purpose better. Given the 80 COCO categories, we can plot a curve for 70 seen \& 10 unseen, 60 seen \& 20 unseen, 50 seen \& 30 unseen, ..., 10 seen \& 70 unseen. If we don't know which 70 seen classes to choose, we just randomly sample 70 seen classes from 80 COCO classes. We can do this random sample 3 times, and report both the average and std for the AR@100 metric.}. \WW{I think Heng has a point here; unless we have time to plot the curve with our method as well, it can raise more questions. We can save this for supp and move to main paragraph when we have better conclusion.}}
%}
%\end{figure}

One may wonder where exactly the gap lies. There are two main types of approaches for instance segmentation popularly used in computer vision literature: bottom-up~\cite{SelectiveSearch,Achanta10slicsuperpixels,GBH,SEEDS3D,StreamGBH} and top-down~\cite{FasterRCNN,8237584,7780460}. Bottom-up approaches are often non-parametric, using local affinities (e.g. similar color or texture) to inform a grouping mechanism which aggregates pixels into regions and instance proposals~\cite{SelectiveSearch}. Top-down approaches are usually high-capacity models, e.g., CNNs, trained end-to-end in a top-down fashion~\cite{8237584} using strong supervision. %from the loss all the way to the pixels. They are implemented by high-capacity models with millions of parameters which are jointly optimized during end-to-end training such as Mask R-CNN~\cite{8237584} or YOLO~\cite{7780460}. 
Bottom-up and top-down approaches have different drawbacks for open-world instance segmentation. Figure~\ref{fig:intro} (b) and (c) show proposals from Selective Search~\cite{SelectiveSearch} (a popular pre-deep-learning bottom-up approach) and Mask R-CNN~\cite{8237584} (a SOTA top-down, closed-world approach) on an image from ADE20K~\cite{8100027}. 
%Selective Search is a bottom-up approach for object proposals which was popularly used before deep learning while Mask R-CNN is a top-down state-of-the-art approach for closed-world instance segmentation. 
%As we can observe, Selective Search makes many small bounding box proposals (Figure~\ref{fig:intro} b) top row) as a result of making independent bottom-up merging decisions. This can also be explained by the fact that Selective Search has no learning, thus it does not have any notion of object boundaries or objectness.
One can see that Selective Search proposes many small boxes (Figure~\ref{fig:intro} b) top row), reflecting the bottom-up merging nature of the method; without stronger instance-level information it is difficult for bottom-up methods to confidently identify coherent object-level predictions.
%\mdf{I don't think the point is object boundaries; it's more that it doesn't have any signal about objectness and does the best it can with local cues}. 
On the other hand, Mask R-CNN is biased towards seen categories learned during training and misses many unseen objects (Figure~\ref{fig:intro} c) top row). It detects only 5 out of 20 ground-truth annotated objects in this example.


\WW{merge below two paragraphs into one}
Here we propose a method which combines the class-agnostic nature of bottom-up local affinity with the object-level coherence provided by top-down approaches. We first learn a local, bottom-up affinity measure from instance masks without their class labels; this provides object-level supervision without explicit coupling to a specific taxonomy. Indeed, we show that this measure generalizes well in out-of-domain evaluation (Figure~\ref{fig:pa_encoding}). We then develop a method to use this affinity measure to construct a large set of pseudo-ground-truth masks; this allows us to expand our mask inventory beyond the original domain(s) of annotation. Finally, we train our Generic Grouping Networks (\Ours{}) end-to-end in a top-down fashion, using both human-annotated, fixed-taxonomy masks and generic, pseudo-GT masks. This significantly improves performance in open-world problems.

We propose to decompose open-world instance segmentation into two parts: a local representation that describes local relationship between neighboring pixels, whether two pixels should be grouped together, and an objectness score by taking a global view of the grouped segments. To implement, we adopt pseudo-ground-truth training paradigm. Given a set of ground truth masks, we first train a Pairwise Affinity predictor (\emph{PA Pred.}) to learn pixel-level pairwise affinities from images (Figure~\ref{fig:overview} a). We then feed predictions from \emph{PA Pred.} to generate pseudo-ground-truth masks through a bottom-up grouping module (Figure~\ref{fig:overview} b). Finally, a generic object proposal network (Figure~\ref{fig:overview} c) is trained with a combination of GT and pseudo-GT masks.

\begin{figure*}
  \centering
    \includegraphics[width=\linewidth]{latex/images/overview.pdf}
  \vspace{-16pt}
  \caption{{\bf An overview of our approach}. (a) First, a Pairwise-Affinity Predictor (\emph{PA Pred.}) is trained to predict pairwise affinities using non-exhaustive segmentation masks as supervision. (b) Once trained, \emph{PA Pred.} is used to predict pairwise affinities of the images. A grouping module is then applied on the predicted pairwise affinity maps to generate pseudo-ground-truth masks. (c) A class-agnostic generic object proposal network (e.g. class-agnostic Mask R-CNN) is trained end-to-end using a combination of GT and generated pseudo-GT masks.}
  \label{fig:overview}
  \vspace{-5pt}
\end{figure*}

Our contributions in this paper include: 
\begin{itemize}
    \item A novel approach, {\bf G}eneric {\bf G}rouping {\bf N}etworks (\Ours{}), for open-world instance segmentation based on learned pixel-level pairwise affinities, bottom-up grouping, and top-down training.
    \item Comprehensive ablation experiments which provide insights about \Ours{} and the problem of open-world instance segmentation.
    \item \Ours{} achieve state-of-the-art performance in open-world instance segmentation on benchmarks including COCO, LVIS, ADE20K, and UVO.
\end{itemize}

==> latex/technical.tex <==
\section{Method}

In this section, we introduce three main components in our approach: learning pairwise affinity, extracting segments from pairwise affinity, leveraging the segments to improve open-world detection performance. 

\subsection{Representing Grouping by Pairwise Affinity}

Pixel grouping is typically represented as segments or masks: pixels belonging to the same group are assigned to the same index. Such representation takes a global view of the grouping of the whole image: pixels are compared globally with all other pixels inside the picture. Learning and predicting such representation gives a rich set of computer vision tasks, such as instance segmentation and panoptic segmentation. However, representing grouping by segments induces strong top-down supervision signals, and thus generalizes poorly when new types of segments (eg. novel objects) are seen. 

On the other hand, grouping can be represented locally, as a pixel-level affinity map. Instead of assigning a single segment index for each pixel belonging a group, grouping of a pixel can be represented by its pairwise affinity with its neighboring pixels, whether these two pixels belong to the same group or not. In the language of instance segmentation, the pairwise affinity of two pixels is 1 if they belong to the same instance, and 0 otherwise. Leveraging the pairwise affinity, one can reconstruct the top-down segment representation in a bottom-up fashion, conditioned on no disconnected part in a segment. 

Specifically, given an RGB image of $3\times H\times W$, its grouping represented by $K$ segments is represented as $K\times H\times W$, where $[k, i, j] = 1$ if pixel ${i, j}$ belongs to segment $k$. The segment representation can be decomposed as a $8\times H\times W$ local representation of pairwise affinity with its $3\times 3$ local neighborhood (8-neighbors). Given pixel ${i, j}$, its $p$th neighbor ($p \in [1, 8]$), $[p, i, j] = 1$ if the pixel and its neighbor belongs to the same instance, and $[p, i, j] = 0$ otherwise. \WW{write this more clear and concise}

Representing grouping by pairwise affinity offers a major advantage: it generalizes better. In other words, the gap between a known object and a novel object is small in their pixel pairwise affinities. \WW{Add qualitative results here}

\subsection{Pairwise Affinity to instance segments}

\subsection{Improving detectors in the open-world}

==> latex/technical_du_edit.tex <==
\section{Open-world instance segmentation}
\label{sec:technical}

We propose a novel approach for open-world instance segmentation by leveraging both low-level bottom-up grouping and top-down supervised training. Figure~\ref{fig:overview} presents an overview of our proposed approach. We first train a Pairwise Affinity predictor (\emph{PA Pred.}) using non-exhaustive segmentation mask annotations to learn pixel-level pairwise affinities from images (Figure~\ref{fig:overview} a). Once trained, \emph{PA Pred.} is used to extract pairwise affinities of the images. The pairwise affinity maps are fed 
to a grouping module to extract pseudo-ground-truth masks (Figure~\ref{fig:overview} b). Finally, a generic object proposal network (Figure~\ref{fig:overview} c) is trained with a combination of GT and pseudo-GT masks.
%the training images with their generated pseudo-truth masks are used to train a generic object proposal network (Figure~\ref{fig:overview} c). 
%As we show later in our experiments
As shown in the experiments (section~\ref{sec:experiments}), this generic object proposal network is useful for open-world instance segmentation.
%and closed-world object segmentation. 
We present each module in the following.
%In the following subsections, we will present each component of our approach in further detail.

\begin{figure*}
  \centering
    \includegraphics[width=\linewidth]{latex/images/overview.pdf}
  \vspace{-16pt}
  \caption{{\bf An overview of our approach}. (a) First, a Pairwise-Affinity Predictor (\emph{PA Pred.}) is trained to predict pairwise affinities using non-exhaustive segmentation masks as supervision. (b) Once trained, \emph{PA Pred.} is used to predict pairwise affinities of the images. A grouping module is then applied on the predicted pairwise affinity maps to generate pseudo-ground-truth masks. (c) A class-agnostic generic object proposal network is trained end-to-end using a combination of GT and generated pseudo-GT masks.}
  \label{fig:overview}
  \vspace{-5pt}
\end{figure*}

\subsection{Learning class-agnostic pairwise affinities}

\noindent {\bf Problem definition}. Given an input image $I \in \mathbb{R}^{3 \times H \times W}$  where $H \times W$ is the image resolution, and $3$ represents the RGB channels. $\mathcal{F}$ is trained to predict the ground-truth pairwise affinities $P$ of the image $I$. Considering the $3\times3$ neighborhood, $P \in \{0,1\}^{8 \times H \times W}$ and $P_{i,j} \in \{0,1\}^8$ encodes the local pixel-level pairwise affinities of the pixel $(i,j)$ with its 8-neighboring pixels in the image $I$. Figure~\ref{fig:pa_encoding}~(c) illustrates the pairwise affinity encodings of the two pixels at the centers of the two image patches marked with the pink and yellow squares in Figure~\ref{fig:pa_encoding}~(a) and (b). Learning is done by minimizing an empirical loss over the training set: % training data:
\begin{equation}
    \min_{\Theta} \sum_i\mathcal{L}(\mathcal{F}(I_i,\Theta), P_i)
\end{equation}
where $\mathcal{F}$ is a non-linear function parametrized by $\Theta$ predicting soft affinities of image $I$, e.g., $\hat{P}=\mathcal{F}(I, \Theta)$. $\hat{P} \in \mathbb{R}^{8 \times H \times W}$ is the predicted pairwise affinities with $\hat{P}_{i,j} \in \mathbb{R}^8$. We note that $\hat{P}_{i,j}$ is not a binary vector, but a real-value one with all of its elements have values in $[0,1]$. In theory, $\mathcal{F}$ can be implemented with any computer vision model that can make pixel-level predictions such as FCN~\cite{fcn} and UPerNet~\cite{UPerNet}.

%\WW{Minor: for notation on PA, should we use ${A}$?}->\DT{PA is more clear/easier to remember to readers}

\noindent {\bf Generate pairwise affinity supervision from non-exhaustive segmentation masks}. Ideally, if all pixels in the image are exhaustively annotated with instance segmentation masks, e.g., all object boundaries are labelled, then all pairs of neighboring pixels can provide good supervision signal for learning pairwise affinity. However, exhaustive annotations for instance segmentation are expensive and time-consuming to obtain, and most datasets come with non-exhaustive segmentation masks. For example, COCO~\cite{Lin2014MicrosoftCC} provides non-exhaustive instance segmentation annotations, thus un-annotated out-taxonomy objects may be (mis-)labelled as background and it is not correct to mark all background neighboring pixels as belonging to the same object. More specifically, we only use neighboring pixels with foreground--foreground or foreground--background relation for training pairwise affinities while ignoring background-background pairs. This can be realized in the following loss:

\begin{equation}
    \mathcal{L}(\hat{P}, P) = \sum_{(i,j) \in I \setminus \mathcal{B}} \ell (\hat{P}_{(i,j)},P_{(i,j)})
\end{equation} \label{equ:loss}
where $\mathcal{B}$ is the set of pixels in the image that fall into background--background group, e.g., the pixels that have all neighboring pixels and itself labelled as background. 

Training of pairwise affinities is unbalanced: among pixels in the image, grouping is common, while separation is rare. Only pixels at an object's boundary has zero-valued affinities, while all other pixels have affinities 1 to all their neighbors. To tackle this problem, we weight the positive affinities by computing the ratio between the positive affinities and negative affinities on a subset of training data, and use the proper weight (e.g., 0.05) for positive predictions.  
% \Heng{I suggest to move the Loss function paragraph in Section 4.2 to here directly.}


\noindent {\bf What does a Pairwise Affinity predictor learn?}
% {\bf Pairwise Affinity predictors do learn to generalize semantic edges}
%\mdf{Du, this paragraph seems to undersell the zebra example.  Perhaps a title that emphasizes that PA actually learns instance edges would help.}\DT{yes, you refer to have a strong statement rather than a question in the header?} 
Intuitively, an ideal PA measure should discriminate between instance boundaries and instance interiors: e.g., if the two neighboring pixels cross an object boundary or not. Ideally, our PA predictor would work across different categories, i.e. it should be robust to all object boundaries, not just the object categories seen during training.  This is a key requirement for success in the open-world setting. Figure~\ref{fig:pa_encoding}~(e) visualizes a pairwise affinity prediction of our PA predictor which is trained using only ground truth masks of only person category from COCO~\cite{Lin2014MicrosoftCC}. It is evident that our PA predictor can learn to generalize to unseen classes such as zebra in this example. We note that `person' masks are particularly diverse owing to clothing and accessories. This is helpful for models to learn and generalize the notion of semantic boundaries. In fact, our PA predictor learns instance boundaries and generalizes well to unseen classes. Figure~\ref{fig:open_image_masks_extended}~(a) visualizes examples of pseudo-GT instance masks generated using a PA predictor trained on only VOC categories. We note that it recovers boundaries for objects such as snake and bear which are clearly out of VOC 20 categories. Finally, we point out that pairwise affinity should capture the semantics of instance boundaries; this is quite different from visual edge maps because many visual edges are not instance boundaries. Figure~\ref{fig:pa_encoding}~(e) presents the edge prediction of the same image predicted by an off-the-shelf edge detector~\cite{soria2020dexined}. This example clearly shows that many visual edges on the back of the zebra are not object boundaries, but are of course still detected by an edge detector.


%Finally, we would like reemphasize that pairwise affinity should carry the semantic of object boundaries and is quite different from conventional edge maps because not all edges are object boundaries. Figure~\ref{fig:pa_encoding}~(e) presents the edge prediction of the same image predicted by an off-the-shelf edge detector~\cite{soria2020dexined}. This example shows that there are many edges on the back of the zebra which are not object boundaries but still be detected by the edge detector.

\begin{figure}
  \centering
    \includegraphics[width=0.96\linewidth]{latex/images/pa_encoding_plus.pdf}
  \vspace{-12pt}
  \caption{{\bf Pairwise affinity encoding and prediction}. Visualization of an example input image (a) and its corresponding ground truth mask annotation (b) and two pairwise-affinity encoding vectors (c) of the two center pixels of the two image patches marked with pink and yellow squares. The pink-patch's center pixel belongs to the same instance with all of its 8-neighbor pixels, thus it is encoded with a vector of all ones. The yellow-patch's center pixel lies at the object boundary and has 4 neighbor pixels belonging to background, thus it is encoded with a binary vector with four 0s and four 1s. (d) Edge prediction of the image in (a) using off-the-shelf edge detector~\cite{soria2020dexined}. (e) Pairwise affinity prediction of the image in (a) using our Pairwise Affinity predictor. Our predictor is trained using only person category masks from COCO. Best viewed in color.}
  \label{fig:pa_encoding}
  \vspace{-8pt}
\end{figure}


\subsection{Pseudo-ground truth mask generation}

\noindent {\bf Grouping pixels into regions}. We now describe how to extract pseudo-truth masks for an image $I$ given a trained PA predictor $\mathcal{F}$. We first obtain the affinity map of the image $I$ by using PA predictor, e.g., $A=\mathcal{F}(I)$. Given the affinity map $A$, there are several ways to group pixels into instances to form mask for each instance. One may use the \emph{Connected Component} (CC) algorithm for grouping. CC treats all affinities independently using a hard cut-off threshold to decide pixel connections which may be a sensitive parameter to tune. Alternatively one may use \emph{graph-based hierarchical} grouping (GBH)~\cite{gb} which is a variant of agglomerative clustering. In segmentation literature~\cite{ArbelaezMFM11,ZhangM20}, Watershed Transform (WT) and Ultrametric Contour Map (UCM)\cite{ucm} are also used for grouping from the edge map of an image. In order to use WT+UCM, we first aggregate the image pairwise affinity map into a semantic edge map using pooling along the channel dimension, e.g., reducing from 8-channels to 1-channel. This semantic edge map is passed to WT+UCM for grouping. We note that Normalized Cut~\cite{ShiM00} can also be used for grouping; however the computational cost is high due to the requirement of solving the associated eigenvalue problem. %We further note that Graph Cut~\cite{BoykovVZ01} is not applicable here because we have no unitary potentials, but only pairwise potentials \mdf{I think it would help to spell out that standard graph-cut approaches to introducing an appearance model would likely be at odds with our learned affinity measure -- or just remove this point unless we get asked. }\DT{agree}. 
We provide the ablation comparing CC, GBH, and WT+UCM in section~\ref{sec:experiments}.

%\mdf{Let's avoid using the 'potential' terminology; we haven't set things up in terms of MRFs and cliques which is where you introduce potential functions.}\DT{true, this terminology is only needed if we want to do Graph Cut approaches.}

\noindent {\bf Ranking and selecting regions}. While connected component algorithm provides a single grouping resulted in non-overlapped regions, GBH and WT+UCM provide a tree defining region hierarchy and thus having possible overlapped regions, e.g., leaf and internal regions. We further use pairwise affinities to define the objectness score of each region $R$ by
\begin{equation}
\mathcal{O}(R) = \frac{Inner(R)}{R_{inner}}-\frac{Outer(R)}{R_{boundary}}
\label{equ:objectness}
\end{equation}
% \mdf{Is this the same as normalized cuts (but with PA)?} \WW{Not exactly the same; NCut is more like (Boundary PA / (Inner PA + Boundary PA)), didn't get a chance to try this but it could be strong.}
where $Inner(R)$ and $Outer(R)$ are the inner and outer affinities %\mdf{call this "total affinity" or similar?} 
of $R$ defined by the sum of pairwise affinities of pixels inside or crossing-boundary of $R$, respectively. $R_{inner}$ and $R_{boundary}$ denote the number of pixels inside $R$ or on the boundary of $R$, respectively. Intuitively, we want to rank high for the mask with strong inner pairwise affinities and weak affinities at the boundary (a.k.a strong cut). Both of inner and outer affinities are normalized the number pixels of the inner mask or at the mask boundary. We use the objectness score defined in Eq.~\ref{equ:objectness} to rank regions provided by grouping methods. We then select only top-k regions from each image as pseudo ground-truth (GT) masks for training our generic object proposal network. Since the whole approach to generate pseudo-GT masks are designed in a bottom-up fashion, we expect the pseudo-GT masks will cover a diverse set of objects and parts, and more importantly most of them are from unseen categories, as shown in Figure~\ref{fig:pa_encoding} we can recover zebra boundary even with a PA predictor trained on person masks.

\subsection{Generic Grouping Networks (\Ours{})}
% \Heng{Not sure we want to give it a new name "Generic Grouping Networks", since the technical difference is small. The reviewers may think we oversell our work here.} Let's keep this for now.
\noindent {\bf Training \Ours{}}. As our PA predictor and grouping module are class-agnostic and can generalize to unseen classes, we apply this bottom-up approach on a large-scale image dataset, e.g., OpenImages~\cite{OpenImages2}, to generate pseudo-GT masks and use them to train a Generic Grouping Network (\Our{}). We note that any architecture for object detection or segmentation, such as Faster R-CNN~\cite{FasterRCNN}, Mask R-CNN~\cite{8237584}, YOLO~\cite{7780460}, or Swin Transformer~\cite{swin_transformer}, can be adopted to train our \Ours{}. The adoption is as simple as making the multi-class classification prediction head into a binary foreground vs. background classification head. For object detection architectures, such as Faster R-CNN~\cite{FasterRCNN} or YOLO~\cite{7780460}, we can easily convert our pseudo-GT masks into boxes for training those detection architectures. Since our \Our{} is trained on a large and diverse set of masks, it is expected to generalize to unseen classes, thus providing a good solution for open-world instance segmentation.

% \noindent {\bf Applications of \Ours{}}. \Our{} can be used for open-world instance segmentation as is (without fine-tuning) since it was trained in a class-agnostic fashion and on a diverse set of pseudo-GT masks. \Ours{} can also be used in traditional closed-world detection or segmentation to replace the proposal part (the grouping module) of the detection or segmentation models. The typical grouping modules are the Selective Search~\cite{SelectiveSearch} in R-CNN~\cite{girshick13} or the Region Proposal Networks (RPNs) in Faster R-CNN~\cite{FasterRCNN} and Mask R-CNN~\cite{8237584}. 

==> latex/wild.tex <==
\begin{figure*}[!]
   \centering
     \includegraphics[width=\linewidth]{latex/images/open_images_masks_extended.pdf}
    \vspace{-12pt}
   \caption{{\bf Pseudo-ground-truth masks generated on OpenImages}. (a) Visualization of some examples from OpenImages with top-5 pseudo-GT masks generated using PA predictor trained on VOC categories. Variety of masks capture persons, objects, and animals. Our PA predictor generalizes well to out-of-taxonomy objects as it retrieves masks for snake and bear which are outside of VOC categories. (b) Performance of \Our{} on ADE20k w.r.t the number of pseudo-GT masks used in pretraining.}
   \label{fig:open_image_masks_extended}
   \vspace{-8pt}
\end{figure*}

\section{Open-world segmentation in the wild}
\label{sec:wild}

Ablation studies in section~\ref{sec:experiments} focus on cross-category generalization in a controlled version of open-world. A more practical question is: how well detectors can generalize across datasets in the wild. It is difficult to evaluate since common datasets, e.g., COCO and LVIS, are only \textit{partially-annotated}. Evaluating open-world segmentation on such datasets may fail to capture performance difference across methods due to punishing precision and not rewarding recall~\cite{Chavali2016ObjectProposalEP}. To handle this, we adopt ADE20k~\cite{8100027} and UVO~\cite{uvo} for evaluating generic proposals in the wild open-world. Specifically, we treat each segmentation mask in ADE20k or UVO as a ground-truth semantic entity and evaluate Average Recall (AR). This setup evaluates both in-taxonomy and out-taxonomy segments. While UVO contains only objects, ADE20k includes also stuff segmentation masks. 
We emphasize that this is truly {\bf in the wild test} as no fine-tuning is done on ADE20k or UVO.  

We compare \Our{} with Selective Search~\cite{SelectiveSearch} and Mask R-CNN baselines trained with the GT masks of (i) 20 VOC classes and (ii) all 80 COCO classes from COCO dataset (Table~\ref{tab:compare_ade}). When trained with the same number of GT masks, \Our{} (enhanced by pseudo masks) significantly outperforms the baseline (\#1 vs.\#2 and \#5 vs.\#6). In addition, we found that \Our{} trained using only VOC masks slightly outperforms the baseline model trained on all 80 COCO category masks (\#2 vs.\#5) on ADE20K, demonstrating its strong performance in the open-world.

% \mdf{It might help to call out that there are no pseudomasks used here, since we've made a big deal about pseudo-masks in the previous sections.} 

% \begin{table}[t]
% \captionsetup{font=footnotesize}
%   \centering
%   {\small
%   \begin{tabular}{|c|c|c|c|c|}
%     \hline
%     GT Masks & Pseudo-GT & AR@100 & AR@300 & AP  \\
%     \hline
%     \multirow{2}{*}{VOC} & None & 11.4 & 15.7 & 4.8 \\
%      & VOC images & \underline{15.1} & \underline{20.3} & \underline{6.7} \\
%      & VOC images & \underline{15.1} & \underline{20.3} & \underline{6.7} \\
%     \hline
%     \multirow{2}{*}{COCO} & Mask R-CNN & 14.7 & 19.8 & 6.4 \\
%      & \Our{} & \textbf{19.2} & \textbf{24.9} & \textbf{8.5} \\
%     \hline
%     \multicolumn{2}{|c|}{OpenImages pseudo} & 13.8 & 18.1 & 4.8 \\
%     \hline
%     \multicolumn{2}{|c|}{+ VOC finetune} & 17.1 & 22.8 & 7.0 \\
%     \hline
%   \end{tabular}}
%   \caption{\textbf{Open-world segmentation in the wild.} \Our{} significantly outperforms the baseline Mask R-CNN when using same amount of training data and annotation. \Our{} trained with masks of only 20 VOC classes still slightly outperforms the baseline trained with masks of full 80 COCO categories. Adding pseudo-GT masks from OpenImages further improves performance. \mdf{This last point isn't clear -- what lines are being compared in the table?}}
%   \label{tab:compare_ade}
% \end{table}

% \begin{table}
% % \captionsetup{font=footnotesize}
%   \centering
%   {\small
%   \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%     \# & PA & GT & Pseudo-GT & AR\footnotesize 100 & AR\footnotesize 300  \\
%     \hline
%     1 & \xmark & VOC & \xmark & 11.4 & 15.7 \\
%     %\hline
%     2 & VOC & VOC & VOC & 15.1 & 20.3 \\
%     %\hline
%     3 & VOC & \xmark & OpenImages & 13.8 & 18.1 \\
%     %\hline
%     4 & VOC & VOC & \footnotesize OpenImages+VOC & \underline{17.1} & \underline{22.8} \\
%     %\hline 
%     5 & \xmark & COCO & \xmark & 14.7 & 19.8 \\
%     %\hline
%     6 & COCO & COCO & COCO & \textbf{19.2} & \textbf{22.5} \\
%     \hline
%     \textcolor{gray}{7} & \multicolumn{3}{c|}{\textcolor{gray}{Selective Search}} & \textcolor{gray}{3.8} & ? \\
%     \hline
%   \end{tabular}}
%   \vspace{-8pt}
%   \caption{\textbf{Open-world segmentation in the wild.} \Our{} significantly outperforms the baseline Mask R-CNN when using same amount of training data and annotation. \Our{} trained with masks of only 20 VOC classes still slightly outperforms the baseline trained with masks of full 80 COCO categories. Adding pseudo-GT masks from OpenImages further improves \Our{} performance. Rows marked with a \xmark in the PA column are baselines.}
%   \label{tab:compare_ade}
% %   \vspace{-5pt}
% \end{table}

\begin{table}
% \captionsetup{font=footnotesize}
  \centering
  {\small
  \begin{tabular}{|c|c|c|c|c|c|}
    \hline
    \# & PA & GT & Pseudo-GT & ADE20k & UVO  \\
    \hline
    1 & \xmark & VOC & \xmark & 11.4 & 32.3 \\
    %\hline
    2 & VOC & VOC & VOC & 15.1 & 36.5 \\
    %\hline
    3 & VOC & \xmark & OpenImages & 13.8 & 25.3 \\
    %\hline
    4 & VOC & VOC & \footnotesize OpenImages+VOC & \underline{17.1} & 38.3 \\
    %\hline 
    5 & \xmark & COCO & \xmark & 14.7 & \underline{40.1} \\
    %\hline
    6 & COCO & COCO & COCO & \textbf{19.2} & \textbf{42.6} \\
    \hline
    \textcolor{gray}{7} & \multicolumn{3}{c|}{\textcolor{gray}{Selective Search}} & \textcolor{gray}{3.8} & \textcolor{gray}{4.7} \\
    \hline
  \end{tabular}}
  \vspace{-8pt}
  \caption{\textbf{Open-world segmentation in the wild on ADE20k and UVO.} \Our{} significantly outperforms the baseline Mask R-CNN when using same amount of training data and annotation. \Our{} trained with masks of only 20 VOC classes still slightly outperforms the baseline trained with masks of full 80 COCO categories on ADE20k. Adding pseudo-GT masks from OpenImages further improves \Our{} performance. Rows marked with a \xmark \ in the PA column are baselines without pseudo-GT. All methods are evaluated by AR@100.}
  \label{tab:compare_ade}
%   \vspace{-5pt}
\end{table}

%\subsection{Training \Our{} with a large-scale unlabeled image dataset}

% \begin{figure*}
% \centering
% \captionsetup{font=footnotesize}
% {\small 
%  \begin{subfigure}[b]{0.75\linewidth}
%     {\includegraphics[width=\linewidth]{./images/open_images_masks.pdf}}
%     \caption{{\bf Pseudo-truth masks generated on OpenImages}. Visualization some examples from OpenImages with top-5 pseudo-grouth-truth masks generated using PA predictor trained on VOC categories. Variety of masks capture persons, objects, and animals.}
%  \end{subfigure}
%  \begin{subfigure}[b]{0.24\linewidth}
%     {\includegraphics[width=\linewidth]{./images/scale_masks.pdf}}
%     \caption{}
%  \end{subfigure}
% %  \caption{{\bf Certain types of data augmentation provide good supervision to pairwise affinities training.} The performance is evaluated by UCM masks generated by the pairwise affinities. Performance is represented as gain (loss) in AR100 compared to without augmentation.  
% %  }
%  \label{fig:open_image_masks}
%  }
% \end{figure*}

%\begin{figure*}
%   \centering
%     \includegraphics[width=0.96\linewidth]{latex/images/open_images_masks_extended.pdf}
%    \vspace{-12pt}
%   \caption{{\bf Pseudo-ground-truth masks generated on OpenImages}. (a) Visualization of some examples from OpenImages with top-5 pseudo-GT masks generated using PA predictor trained on VOC categories. Variety of masks capture persons, objects, and animals. Our PA predictor generalizes well to out-of-taxonomy objects as it retrieves masks for snake and bear which are outside of VOC categories. (b) Performance of \Our{} on ADE20K w.r.t the number of pseudo-GT masks used in pretraining.}
%   \label{fig:open_image_masks_extended}
%\end{figure*}

Since PA-based bottom-up grouping can generate masks for any unlabelled images, we further hypothesize that training with additional pseudo-GT masks helps open-world segmentation. To test, we use the PA predictor trained \textbf{only} on VOC-category masks in COCO and extract pseudo-GT masks from 100k randomly sampled images from OpenImagesV4~\cite{OpenImages} to train downstream detectors. We visualize some of images with their top-5 pseudo masks in Figure~\ref{fig:open_image_masks_extended}~a.

\noindent {\bf Using more pseudo-GT masks improves open-world segmentation}. On the same 100k images from OpenImages, we vary the number of pseudo-GT masks used for training \Our{} by selecting top-k masks per image (e.g., $k=1,3,5,10,20$). We found that using more pseudo-GT masks improves AR@100 by $1.6\%$ (Figure~\ref{fig:open_image_masks_extended}~b.). Training with only pseudo-mask (\#3) outperforms training with human-annotated VOC masks (\#1) by +2.4\% on ADE20k. We further finetune the detector on VOC GT masks and pseudo masks generated and improves the performance (\#4). We refer readers to supplementary materials for more studies on scaling experiments of unlabeled images.

% {\bf Using only pseudo-GT masks outperforms baselines and reaches upper bound}

% {\bf Using only pseudo-GT masks together with GT masks further improves}

% \textbf{More masks improve detector recall.} We observe a promising trend as we increase the number of masks: using more pseudo masks used improves detector's recall (Fig.~\ref{fig:open_image}.). Even with 20 masks per image sampled, it does not hurt detector performance compared with 10 masks per image. In fact, with 20 masks sampled per image, \Our{} outperforms Mask R-CNN trained on human-annotated VOC masks (same masks pairwise affinities are trained) by 2.4\% (Table~\ref{tab:compare_ade}) and is only 0.9\% below Mask R-CNN trained on full COCO masks.  

%\begin{figure}
%\centering
%\captionsetup{font=footnotesize}
%{\small 
% \begin{subfigure}[b]{0.65\linewidth}
%    {\includegraphics[width=\linewidth]{./images/scale_masks.pdf}}
    % \caption{}
% \end{subfigure}
%  \begin{subfigure}[b]{0.49\linewidth}
%     {\includegraphics[width=\linewidth]{./images/image_net_pretrain.pdf}}
%     \caption{}
%  \end{subfigure}
% \caption{{\bf Evaluation of detectors trained with pseudo-masks generated on OpenImages}. We ablate on the number of masks generated to train \Our{} using only 100k images from OpenImages. We take top-k masks per image, where k equals to [1, 3, 5, 10, 20]. We observe a promising trend as we increase number of masks. %(b) We compare detectors initialized with / without ImageNet pretrained backbone, then further trained with our pseudo masks generated on subset of OpenImages with increasing size. With 750k images from OpenImages, the detector (initialized with random weights) reaches the same AR100 with model pretrained on ImageNet.
% }
% \label{fig:open_image}
% }
%\end{figure}


 
% \begin{figure}
%   \centering
%     \includegraphics[width=\linewidth]{latex/images/scale_masks.pdf}
%   \caption{{\bf Scaling number of masks with pseudo mask improve recall in the open-world}. We ablate on the number of masks generated to train \Our{}. We take top-k masks per image, where k equals to [1, 3, 5, 10, 20]. We observe a promising trend as we increase number of masks.}
%   \label{fig:scale_mask}
% \end{figure}

%\textbf{Is ImageNet pretraining necessary?} Pairwise affinities can generate pseudo masks with human annotations at scale\DT{I don't understand this sentence}, and we revisit whether ImageNet pre-training is necessary in this setup. In Figure~\ref{fig:open_image}~b, we show that \Our{} performs competitively with ImageNet pretrained model on Recall, although performs worse on Precision. This suggests that out model benefits more from ImageNet pre-training on \textit{ranking} the segments and less on \textit{producing} the segments. \mdf{These results don't feel fully-baked enough to be discussing here; can we remove this experiment?}\DT{yes, we will remove this setup}

% \textbf{As pre-training for \Our{}.} We pretrain \Our{} by pseudo masks of OpenImages and finetune on VOC masks plus pseudo-GT masks on COCO images. This can further improve AR@100 from 15.1\% (Table~\ref{tab:compare_ade}) to 17.1\%.

